Improving the HardNet Descriptor

In the thesis we consider the problem of local feature descriptor learning for wide baseline stereo focusing on the HardNet descriptor, which is close to state-of-the-art. AMOS Patches dataset is introduced, which improves robustness to illumination and appearance changes. It is based on registered images from selected cameras from the AMOS dataset. We provide recommendations on the patch dataset creation process and evaluate HardNet trained on data of different modalities. We also introduce a dataset combination and reduction methods, that allow comparable performance on a significantly smaller dataset. HardNet8, consistently outperforming the original HardNet, benefits from the architectural choices made: connectivity pattern, final pooling, receptive field, CNN building blocks found by manual or automatic search algorithms -- DARTS. We show impact of overlooked hyperparameters such as batch size and length of training on the descriptor quality. PCA dimensionality reduction further boosts performance and also reduces memory footprint. Finally, the insights gained lead to two HardNet8 descriptors: one performing well on a variety of benchmarks -- HPatches, AMOS Patches and IMW Phototourism, the other is optimized for IMW Phototourism.

==> Tabs/IMW.tex <==
% \definecolor{light-gray}{gray}{0.9}
% \renewcommand{\arraystretch}{0.95}
% \renewcommand{\tabcolsep}{0.8mm}
\begin{table}
\begin{center}
% \begin{adjustbox}{width=\linewidth,center}
\footnotesize
\begin{tabular}{lcccc}
\toprule
Method & Stereo 2k & Stereo 8k\\
\midrule
CV-SIFT & .2875 & .4584 \\
% VL-SIFT & &.4655  \\
% VL-Hessian-SIFT && .4450  \\
% VL-DoGAff-SIFT & & .4680 \\
% VL-HesAffNet-SIFT & & .4679 \\
% \midrule
CV-$\sqrt{\text{SIFT}}$ & .3149 & .4930 \\
%CV-SURF & .2086 & .2593 & .4184 & .4846 \\
%CV-AKAZE &  .2144 & .3074 & .4361 & .5553\\
%CV-ORB & .0819 & .1674 & .1914 & .3509 \\
%CV-FREAK & .1761 & .2711 & .3297 & .4653 \\
\midrule
D2-Net (SS) & .1355& .2228  \\
D2-Net (MS) & .1813 & .2506\\
\midrule
%L2-Net &.3752 & .5295 & .5392 & 6644 \\
% DoG-HardNetAmos+ & & .5385 \\
%Key.Net-HardNet &.4139  & .4986 & .6161 & .6483 \\
DoG-GeoDesc & .3662 & .5111  \\
ContextDesc & .3510& .5098  \\
DoG-SOSNet & .3976 & .5587  \\
DoG-LogPolarDesc & 4115& .5340\\
DoG-HardNet & \bf{.4029}& .5543 \\
\midrule
DoG-HardNet8-PT (ours)  &.3865    &.\bf{5758} \\
DoG-HardNet8-Univ (ours) &.3704    & .5622 \\
%\midrule
%DoGUpright-HardNet &  .4423 & .5727  \\
%\midrule
%DoGUpright-HardNetPT (ours)  &.4446   & .5840 \\
%DoG-HardNetUniv (ours) & .4293    & .5707 \\
%
%
%
%CV-SIFT & .2875 & .4584 & .4562 & .6261 \\
% VL-SIFT & &.4655  \\
% VL-Hessian-SIFT && .4450  \\
% VL-DoGAff-SIFT & & .4680 \\
% VL-HesAffNet-SIFT & & .4679 \\
% \midrule
%CV-$\sqrt{\text{SIFT}}$ & .3149 & .4930 & .4995 & .6765 \\
%CV-SURF & .2086 & .2593 & .4184 & .4846 \\
%CV-AKAZE &  .2144 & .3074 & .4361 & .5553\\
%CV-ORB & .0819 & .1674 & .1914 & .3509 \\
%CV-FREAK & .1761 & .2711 & .3297 & .4653 \\
%\midrule
%%L2-Net &.3752 & .5295 & .5392 & 6644 \\
%DoG-HardNet & .4029& .5543 & .5661 & .7096 \\
% DoG-HardNetAmos+ & & .5385 \\
%Key.Net-HardNet &.4139  & .4986 & .6161 & .6483 \\
%DoG-GeoDesc & .3662 & .5111 &  .5244 & .6803 \\
%ContextDesc & .3510& .5098 & .5568 & .7035 \\
%DoG-SOSNet & .3976 & .5587 & .5784 & .7021 \\
%DoG-LogPolarDesc & 4115& .5340 & .5849 & .6928\\
%\midrule
%D2-Net (SS) & .1355& .2228 & .3943 & .4598 \\
%D2-Net (MS) & .1813 & .2506 & .3007 & .4751\\
%\midrule
%DoGUpright-HardNet & {\bf .4423}& .5727 & .6227 & .7230 \\
%\midrule
%DoG-HardNetPT (ours) &  &  & - &in progress \\
%DoG-HardNetUniv (ours) &  &  & - &in progress \\
%DoGUpright-HardNet (ours) & .4410  & {\bf .5812} & - & .7174 \\
%Key.Net-HardNet (ours) & .4391 & - & .6134 & - \\
% R2D2 (wasf-n8-big) &  & .4437 \\
\bottomrule
\end{tabular}
% \end{adjustbox}
\end{center}
\caption{Mean average precision mAA(10$\degree$) evaluated for the listed models on the IMW Phototourism benchmark.}
\label{tab:IMW}
\end{table}

==> Tabs/nviews.tex <==


\begin{table}[htb]
\centering
\caption[Evaluation of AMOS Views variants.]{Evaluation of AMOS Views variants. mAP measure is evaluated on HPatches if we train HardNet architecture on increasingly larger dataset.}

\begin{tabular}{lccc}
\toprule
Arch $\setminus$ \#Views & 27 & 33 & 52 \\
\midrule

HardNet & 58.48 & 58.27 & 57.71 \\
HardNet8 & 61.47 & 62.00 & 61.30 \\
HardNet8x2 & 62.22 & 62.62 & 62.42 \\
\bottomrule
\end{tabular}
\label{tab:nviews}
   
\end{table}



==> Tabs/results_old.tex <==


\begin{table}[htb]
\centering
\caption{HPatches matching scores (mAP).}

\begin{tabular}{lccc}
    \toprule
    Training set &\multicolumn{3}{c}{HPatches subset}\\
    & illum & view & full \\
    \midrule
  Liberty & 49.86 & 55.62 & 52.79 \\
  6Brown & 52.39 & 59.15 & 55.83 \\
  PS & 48.55 & \textbf{67.43} & 58.16 \\
  \midrule
  Webcam~\cite{Verdie2015} & 51.82 & 50.77 & 51.29 \\
  AMOS-patches  & 55.17 & 57.94 & 56.58\\
  +Liberty & 56.14 & 60.27& 58.24 \\
  +6Brown & \textbf{56.22} & 61.50& \textbf{58.91}  \\
%      ++ & 57.06 & 52.70 & 61.26 \\
    \bottomrule
    
\end{tabular}
\label{tab:results1}
\end{table}



==> Tabs/softmargin.tex <==


\begin{table}[htb]
\centering
\caption[Evaluation of hard margin and dynamic soft margin.]{Evaluation of hard margin and dynamic soft margin. For HPatches and AMOS Patches we measure mean average precision (mAP). In the IMW PT benchmark, validation set, the measure is mean average accuracy, mAA(10\degree).}
   
\begin{tabular}{lccc}
\toprule
Margin & HPatches & AMOS Patches & IMW PT \\
\midrule

Hard & \textbf{52.96} & \textbf{44.21} & \textbf{68.17} \\
Dynamic Soft & 52.83 & 43.99 & 67.87 \\
\bottomrule

\end{tabular}
\label{tab:softmargin}
\end{table}



==> Tabs/wxbstable.tex <==


\begin{table*}[htb]
\centering
\caption{Comparison of HardNet(ours) vs HardNet++~\cite{mishchuk2017working} following the protocol~\cite{wxbs2015}. The number of matched image pairs is shown. The \fbox{numbers} of image pairs in a dataset are boxed. Best results are in \textbf{bold}.}
% \caption{Comparison of the AMOS+6Br HardNet vs. HardNet++~\cite{mishchuk2017working} following the protocol~\cite{wxbs2015}. The number of matched image pairs is shown. The \fbox{numbers} of image pairs in a dataset are boxed. Best results are in \textbf{bold}.}

\setlength{\tabcolsep}{4pt}

\begin{tabular}{lccccccc}
\toprule

&\rotatebox{90}{EF~\cite{Zitnick2011}}
&\rotatebox{90}{EVD~\cite{mishkin2015mods}}
&\rotatebox{90}{OxAff~\cite{Mikolajczyk2005}}
&\rotatebox{90}{SymB~\cite{Hauagge2012}}
&\rotatebox{90}{GDB~\cite{yang2007registration}}
&\rotatebox{90}{map2photo~\cite{wxbs2015}}
&\rotatebox{90}{LTLL~\cite{Fernando2015}} \\

Descriptor
&\fbox{33}
&\fbox{15}
&\fbox{40}
&\fbox{46}
&\fbox{22}
&\fbox{6}
&\fbox{172} \\
 
% \cmidrule(r){1-8}
\midrule

HardNet++~\cite{mishchuk2017working}
& 31& \textbf{15}&\textbf{40} &40 &18 &2& \textbf{108} \\

% HardNetAMOS+6Br
% &\textbf{33} &\textbf{15} &\textbf{40}   &\textbf{45} &\textbf{19} &\textbf{4}&106  \\

HardNet(ours)
\\

\bottomrule
\end{tabular}
\label{tab:wxbs-table}

\end{table*}



==> ctuth-core.tex <==

%!TEX ROOT = ctutest.tex

\ProvidesExplFile{ctuth-core.tex}%
	{2016/06/15}{0.1 t1606152353}%MY TIMESTAMP HERE {0.1}
	{"Core"\space part\space of\space the\space class\space ctuthesis}


%%% GENERAL LaTeX3 THINGIES

\cs_generate_variant:Nn \keys_set:nn { nx }
\cs_generate_variant:Nn \tl_if_eq:nnTF { xn }
\cs_generate_variant:Nn \seq_gconcat:NNN { cc }
\cs_generate_variant:Nn \str_if_eq:nnTF { xn }

\skip_new:N \g_ctuthesis_tempa_skip


%%% CLASS SETUP, FIELDS, TEMPLATES, THEMES

% Set allowed languages: No other languages can ever be main, title or second
\tl_gset:Nn \g_ctuthesis_alllanguages_tl {{czech}{english}{slovak}}

% Error message for using \ctuprocess twice
\msg_new:nnn { ctuthesis } { ctuprocess-twice } { The~macro~ \token_to_str:N \ctuprocess\ should~
	be~used~only~once~in~preamble. }

% Error message for not using \ctuprocess at all
\msg_new:nnn { ctuthesis } { ctuprocess-none } { It~is~necessary~to~use~the~
	macro~ \token_to_str:N \ctuprocess\ once~in~the~preamble. }


%%% KEY-VALUE SETUP

% Two seqs: one for keys that need disabling after \documentclass,
% another one for keys that need disabling after \ctuprocess
\seq_new:N \g_ctuthesis_keys_nop_seq
\seq_new:N \g_ctuthesis_keys_nopost_seq
% Add the clist #2 into seq #1
\cs_new_protected:Nn \ctuthesis_keys_add_no:nn {
	\group_begin:
	\seq_set_from_clist:Nn \l_temp_ctuthesis_a_seq { #2 }
	\seq_gconcat:ccN { g_ctuthesis_keys_#1_seq } { g_ctuthesis_keys_#1_seq } \l_temp_ctuthesis_a_seq
	\group_end:
}

% Error messages for the keyvalue interface
\msg_new:nnn { ctuthesis } { keys-unknown } { The~key~'#1'~is~not~known~to~the~
	class~'ctuthesis'~and~will~be~ignored. }

\msg_new:nnn { ctuthesis } { keys-nopost } { The~key~'#1'~is~forbidden~after~
	\token_to_str:N \ctuprocess \space and~will~be~ignored.~You~may~wish~to~
	set~it~up~before. }

\msg_new:nnn { ctuthesis } { keys-nop } { The~key~'#1'~is~forbidden~in~
	\token_to_str:N \ctusetup \space and~will~be~ignored.~Use~the~optional~argument~
	of~ \token_to_str:N \documentclass \space to~set~it~up. }

% Very standard unknown key treatment
\keys_define:nn { ctuthesis } {
	unknown .code:n = \msg_error:nnx { ctuthesis } { keys-unknown } { \l_keys_key_tl },
}

% Disables keys marked '#1' (either 'nop' or 'nopost')
\cs_new_protected:Nn \ctuthesis_disable_keys:n {
	\seq_map_inline:cn { g_ctuthesis_keys_#1_seq } {
		\keys_define:nn { ctuthesis } {
			##1 .code:n = \msg_error:nnx { ctuthesis } { keys-#1 } { ##1 },
		}
	}
}

% General keys
\tl_gset:Nn \g_ctuthesis_fontsize_tl {11pt}
\seq_new:N \g_ctuthesis_languages_seq
\keys_define:nn { ctuthesis } {
	
	% Only 11pt fontsize is allowed
	fontsize .choices:nn = { 11pt } { \tl_gset_eq:NN \g_ctuthesis_fontsize_tl \l_keys_choice_tl },
	
	% Oneside option
	oneside .bool_gset:c = { g_ctuthesis_switch_oneside_bool },
	oneside .initial:n = { false },
	twoside .meta:n = { oneside = false },
	
	% Draft option
	draft .bool_gset:c = { g_ctuthesis_switch_draft_bool },
	draft .initial:n = { false },
	
	% We use three languages:
	% main for the work itself, ToC and LoFT
	mainlanguage .choice:,
	% title for the titlepage, thanks, declaration and abstract
	titlelanguage .choice:,
	% second is the language of second abstract. First abstract is in title language,
	% second abstract is either in main language, or in English for Czech/Slovak theses
	% or Czech for English theses. It will be set automatically.
	secondlanguage .choice:,

	% otherlanguages will be simply passed on to babel
	otherlanguages .code:n =
		\seq_set_from_clist:Nn \l_temp_ctuthesis_a_seq { #1 }
		\seq_gconcat:NNN \g_ctuthesis_languages_seq \g_ctuthesis_languages_seq \l_temp_ctuthesis_a_seq
		,

}

\ctuthesis_keys_add_no:nn { nop } { draft, fontsize, oneside, twoside }
\ctuthesis_keys_add_no:nn { nopost } { mainlanguage, titlelanguage, secondlanguage }

% Switches defaulting to false
\tl_map_inline:nn { {front-specification}{monochrome}{savetoner}{pkg-listings}{layout-short} } {
	\keys_define:nn { ctuthesis } {
		#1 .bool_gset:c = { g_ctuthesis_switch_#1_bool },
		#1 .initial:n = { false },
	}
}
\ctuthesis_keys_add_no:nn { nopost } { monochrome, savetoner, pkg-listings }

% Switches defaulting to true
\tl_map_inline:nn { {front-list-of-tables}{front-list-of-figures}{pkg-hyperref}{pkg-makeidx}{pkg-amsthm} } {
	\keys_define:nn { ctuthesis } {
		#1 .bool_gset:c = { g_ctuthesis_switch_#1_bool },
		#1 .initial:n = { true },
	}
}
\ctuthesis_keys_add_no:nn { nopost } { pkg-hyperref, pkg-makeidx }

% We allow the key 11pt along with the key fontsize
\tl_map_inline:nn { {11pt} } {
	\keys_define:nn { ctuthesis } {
		#1 .meta:n = { fontsize = #1 },
	}
	\ctuthesis_keys_add_no:nn { nop } { #1 }
}

% Basic fields that are not language-dependent
\tl_map_inline:nn { {author}{supervisor}{supervisor-specialist}{supervisor-address}{day}{month}{year}
	  {facultynum}{specification-file}{preprint} } {
	\keys_define:nn { ctuthesis } {
		#1 .tl_gset:c = { g_ctuthesis_field_#1_tl },
	}
}

% Language-dependent keys and environments
\tl_map_inline:Nn \g_ctuthesis_alllanguages_tl {
	% Various fields in various languages
	\tl_map_inline:nn { {title}{subtitle}{university}{university-endl}{faculty}{department}
		  {doctype}{fieldofstudy}{subfieldofstudy}{keywords} } {
		\keys_define:nn { ctuthesis } {
			##1-#1 .tl_gset:c = g_ctuthesis_field_##1_#1_tl,
		}
	}
	% Sets up the choice for each of the languages
	\tl_map_inline:nn { {mainlanguage}{titlelanguage}{secondlanguage} } {
		\keys_define:nn { ctuthesis } {
			##1 / #1 .code:n =
				\tl_gset:cn { g_ctuthesis_field_##1_tl } { #1 }
				\seq_gput_right:Nn \g_ctuthesis_languages_seq { #1 },
		}
	}
	% The abstract is now language-dependent
	\NewEnviron { abstract-#1 } { \tl_gset:cV { g_ctuthesis_field_abstract_#1_tl } \BODY }
	\tl_new:c { g_ctuthesis_field_abstract_#1_tl }
}

% "abstract" itself is not used, the language of the abstract has to be specified
\msg_new:nnn { ctuthesis } { abstract-forbidden } { The~environment~'abstract'~should~be~replaced~
	by~'abstract-lang'~with~the~proper~language~specified. }
\DeclareDocumentEnvironment{ abstract }{ }{ \msg_error:nn { ctuthesis } { abstract-forbidden } }{ }

% "thanks" and "declaration" are fields, but set up as environments rather then KVs
\cs_undefine:c { thanks }
\NewEnviron { thanks } { \tl_gset:cV { g_ctuthesis_field_thanks_tl } \BODY }
\tl_new:c { g_ctuthesis_field_thanks_tl }
\NewEnviron { declaration } { \tl_gset:cV { g_ctuthesis_field_declaration_tl } \BODY }
\tl_new:c { g_ctuthesis_field_declaration_tl }

\tl_gset:Nn \g_ctuthesis_ctulstbg_tl { ctulstbg }
\keys_define:nn { ctuthesis } {
		ctulstbg .tl_gset:N = \g_ctuthesis_ctulstbg_tl
}


% A macro called after every \keys_set{ctuthesis}{...}
\cs_new_protected:Nn \ctuthesis_ctusetup_trigger: {
	% Remove duplicates from the language list
	\seq_gremove_duplicates:N \g_ctuthesis_languages_seq
	% Set up titlelanguage as mainlanguage if the latter is defined and the former is not
	\bool_if:nT { \tl_if_exist_p:c { g_ctuthesis_field_mainlanguage_tl }
		&& ! \tl_if_empty_p:c { g_ctuthesis_field_mainlanguage_tl }
		&& ( ! \tl_if_exist_p:c { g_ctuthesis_field_titlelanguage_tl }
			|| \tl_if_empty_p:c { g_ctuthesis_field_titlelanguage_tl } )
	} {
		\keys_set:nx { ctuthesis } { titlelanguage = \tl_use:c { g_ctuthesis_field_mainlanguage_tl } }
	}
	% Set up secondlanguage if it has not been set up before
	\bool_if:nT { \tl_if_exist_p:c { g_ctuthesis_field_mainlanguage_tl }
		&& \tl_if_exist_p:c { g_ctuthesis_field_titlelanguage_tl }
		&& ( ! \tl_if_exist_p:c { g_ctuthesis_field_secondlanguage_tl }
			|| \tl_if_empty_p:c { g_ctuthesis_field_secondlanguage_tl } )
	} {
		\tl_if_eq:ccTF { g_ctuthesis_field_mainlanguage_tl } { g_ctuthesis_field_titlelanguage_tl } {
			\tl_if_eq:xnTF { \tl_use:c { g_ctuthesis_field_mainlanguage_tl } } { english } {
				\keys_set:nn { ctuthesis } { secondlanguage = czech }
			} {
				\keys_set:nn { ctuthesis } { secondlanguage = english }
			}
		} {
			\keys_set:nx { ctuthesis } { secondlanguage = \tl_use:c { g_ctuthesis_field_mainlanguage_tl } }
		}
	}
}

% Key setup to be used in the preamble
\NewDocumentCommand \ctusetup { m } {
	\keys_set:nn { ctuthesis } { #1 }
	\ctuthesis_ctusetup_trigger:
}


%%% THEMES, TEMPLATES AND FIELDS

% Theme, template and field hadling - "unknown" error messages
\msg_new:nnn { ctuthesis } { unknown-theme } { Theme~'#1'~has~not~been~defined~
	for~use~with~ \token_to_str:N \ctutheme . }

\msg_new:nnn { ctuthesis } { unknown-template } { Template~'#1'~has~not~been~defined~
	for~use~with~ \token_to_str:N \ctutemplate . }

\msg_new:nnn { ctuthesis } { unknown-field } { Field~'#1'~has~not~been~defined~
	for~use~with~ \token_to_str:N \ctufield . }

% Theme and template hadling - setters
\NewDocumentCommand \ctuthemeset { >{\TrimSpaces}m +m } {
	\cs_set:cn { ctuthesis_theme_#1_var: } { #2 }
}

\NewDocumentCommand \ctutemplateset { >{\TrimSpaces}m +m } {
	\cs_set:cn { ctuthesis_template_#1_var: } { #2 }
}

% Theme, template and field hadling - getters
\NewDocumentCommand \ctutheme { >{\TrimSpaces}m } {
	\cs_if_exist_use:cF { ctuthesis_theme_#1_var: } { \msg_error:nnx { ctuthesis } { unknown-theme } { #1 } }
	}

\NewDocumentCommand \ctutemplate { >{\TrimSpaces}m } {
	\cs_if_exist_use:cF { ctuthesis_template_#1_var: } { \msg_error:nnx { ctuthesis } { unknown-template } { #1 } }
	}

% `\ctufield` supports the context language specifier as an optional argument
\NewDocumentCommand \ctufield { s >{\TrimSpaces}o >{\TrimSpaces}m } {
	\IfBooleanTF { #1 } {
		\IfValueTF { #2 } {
				\ctuthesis_field_use_default:nnn { #2 } { #3 } { }
		} {
				\ctuthesis_field_use_default:nn { #3 } { }
		}
	} {
		\IfValueTF { #2 } {
				\ctuthesis_field_use:nn { #2 } { #3 }
		} {
				\ctuthesis_field_use:n { #3 }
		}
	}
}

% Four variants of the "field use": expandable (with default value)/non-expandable (with error message) and language-independent/dependent
% #1->field, #2->default value
\cs_new:Nn \ctuthesis_field_use_default:nn {
	\cs_if_exist_use:cF { g_ctuthesis_field_#1_tl } { #2 }
}

% #1->language, #2->field, #3->default value
\cs_new:Nn \ctuthesis_field_use_default:nnn {
	\ctuthesis_field_use_default:nn
		{ #2_\ctuthesis_field_use_default:nn { #1 language } { nolanguage } }
		{ #3 }
}

% #1->field
\cs_new_protected:Nn \ctuthesis_field_use:n {
	\cs_if_exist_use:cF { g_ctuthesis_field_#1_tl } { \msg_error:nnx { ctuthesis } { unknown-field } { #1 } }
}

% #1->language, #2->field
\cs_new_protected:Nn \ctuthesis_field_use:nn {
	\cs_if_exist:cTF { g_ctuthesis_field_#1language_tl }
		{ \ctuthesis_field_use:n { #2_\ctuthesis_field_use_default:nn { #1 language } { } } }
		{ \msg_error:nnx { ctuthesis } { unknown-field } { #1 language } }
}

% Theme, template and field hadling - existance conditionals
\prg_new_conditional:Nnn \ctuthesis_theme_exists:n { p, T, F, TF } {
	\cs_if_exist:cTF { ctuthesis_theme_#1_var } { \prg_return_true: } { \prg_return_false: }
}

\prg_new_conditional:Nnn \ctuthesis_template_exists:n { p, T, F, TF } {
	\cs_if_exist:cTF { ctuthesis_template_#1_var } { \prg_return_true: } { \prg_return_false: }
}

\prg_new_conditional:Nnn \ctuthesis_field_exists:n { p, T, F, TF } {
	\cs_if_exist:cTF { g_ctuthesis_field_#1_tl } { \prg_return_true: } { \prg_return_false: }
}

% Theme, template and field hadling - publicly available conditionals with "true" and "false" branches
\DeclareDocumentCommand \ctuiftheme { s >{\TrimSpaces}m +m +m } {
	\ctuthesis_theme_exists:nTF { #2 } {
		\IfBooleanTF { #1 } {
			\tl_if_empty:cTF { g_ctuthesis_theme_#1_tl } { #4 } { #3 }
		} {
			#3
		}
	} {
		#4
	}
}

\DeclareDocumentCommand \ctuiftemplate { s >{\TrimSpaces}m +m +m } {
	\ctuthesis_template_exists:nTF { #2 } {
		\IfBooleanTF { #1 } {
			\tl_if_empty:cTF { g_ctuthesis_template_#1_tl } { #4 } { #3 }
		} {
			#3
		}
	} {
		#4
	}
}

% The starred variant checks for emptiness rather than for existance
\DeclareDocumentCommand \ctuiffield { s >{\TrimSpaces}o >{\TrimSpaces}m +m +m } {
	\IfValueTF { #2 } {
		\ctuthesis_field_exists:nF { #2 language } { \msg_error:nnx { ctuthesis } { unknown-field } { #1 } }
		\IfBooleanTF { #1 } {
			\ctuiffield * { #3_\ctuthesis_field_use:n { #2 language } } { #4 } { #5 }
		} {
			\ctuiffield { #3_\ctuthesis_field_use:n { #2 language } } { #4 } { #5 }
		}
	} {
		\ctuthesis_field_exists:nTF { #3 } {
			\IfBooleanTF { #1 } {
				\tl_if_empty:cTF { g_ctuthesis_field_#3_tl } { #5 } { #4 }
			} {
				#4
			}
		} {
			\ctuthesis_field_exists:nTF { #3 } { #5 } { #4 }
		}
	}
}

% We don't do any check for existance of a switch, so better be careful.
\prg_new_conditional:Nnn \ctuthesis_if_switch:n { p, T, F, TF } {
	\bool_if:cTF { g_ctuthesis_switch_#1_bool } { \prg_return_true: } { \prg_return_false: }
}

\DeclareDocumentCommand \ctuifswitch { >{\TrimSpaces}m +m +m } {
	\bool_if:cTF { g_ctuthesis_switch_#1_bool } { #2 } { #3 }
}


%%% LOGGING

% Create \ctuverlog which contains the automatically updated timestamp of the file.
% It can be used for instance in \ctusetup{preprint = \ctuverlog} in order to show
% the timestamp on every page.
\cs_new_protected:Npx \ctuverlog {
	ctuthesis ~ \use_ii:nn
	{2016/06/15}{ t1606152353}%MY TIMESTAMP HERE {}	
}


\endinput


==> ctuth-names.tex <==

%!TEX ROOT = ctutest.tex

\ProvidesExplFile{ctuthesis-names.def}{2014/01/18}{0.1}{"Names" part of the class ctuthesis}

% This code provides all language-dependent definitions that are needed.
% That is, no "real text" should appear anywhere else.

% We stick to the LaTeX2e syntax here for what's related directly to package `babel`
% Also, we don't use utf8, because if someone decided to switch encodings, they can,
% and we won't prevent them from doing so if we don't have to.

% General titles
\def\ctucaptionsenglish{
	\def\appendicesname{Appendices}
	\def\thanksname{Acknowledgements}
	\def\declarationname{Declaration}
	\def\listfigurename{Figures}
	\def\listtablename{Tables}
	\def\supervisorname{Supervisor}
	\def\supervisorspecialistname{Supervisor--specialist}
	\def\fieldofstudyname{Field\ of\ study}
	\def\subfieldofstudyname{Subfield}
	\def\specificationname{Project\ Specification}
	\def\keywordsname{Keywords}
	\def\titletranslationname{Title\ translation}
}

\def\ctucaptionsczech{
	\def\appendicesname{P\v r\'ilohy}
	\def\thanksname{Pod\v ekov\'an\'i}
	\def\declarationname{Prohl\'a\v sen\'i}
	\def\listfigurename{Obr\'azky}
	\def\listtablename{Tabulky}
	\def\supervisorname{\v Skolitel}
	\def\supervisorspecialistname{\v Skolitel--specialista}
	\def\fieldofstudyname{Obor}
	\def\subfieldofstudyname{Zam\v e\v ren\'i}
	\def\specificationname{Zad\'an\'i\ pr\'ace}
	\def\keywordsname{Kl\'i \v cov\'a\ slova}
	\def\titletranslationname{P\v reklad\ n\'azvu}
}

\def\ctucaptionsslovak{
	\def\appendicesname{Pr\'i lohy}
	\def\thanksname{Po\v dakovanie}
	\def\declarationname{Prehl\'asenie}
	\def\listfigurename{Obr\'azky}
	\def\listtablename{Tabu\v lky}
	\def\figurename{Obr\'azok}
	\def\supervisorname{\v Skolite\v l}
	\def\supervisorspecialistname{\v Skolite\v l--specialista}
	\def\fieldofstudyname{Odbor}
	\def\subfieldofstudyname{Zameranie}
	\def\specificationname{Zad\'an\'i\ \ pr\'ace}
	\def\keywordsname{K\v l\'u\v cov\'e\ slov\'a}
	\def\titletranslationname{Preklad\ n\'azvu}
}

% Name of the university
\ctusetup{
	university-endl-czech = {\v Cesk\'e\\ vysok\'e \\ u\v cen\'i  ~ technick\'e \\ v ~ Praze},
	university-endl-slovak = {\v Cesk\'e\\ vysok\'e \\ u\v cen\'i  ~ technick\'e \\ v ~ Praze},
	university-endl-english = {Czech\\ Technical \\ University \\ in ~ Prague},
	university-czech = {\v Cesk\'e ~ vysok\'e ~ u\v cen\'i  ~ technick\'e ~ v ~ Praze},
	university-slovak = {\v Cesk\'e ~ vysok\'e ~ u\v cen\'i  ~ technick\'e ~ v ~ Praze},
	university-english = {Czech ~ Technical ~ University ~ in ~ Prague},
}

% Month names handling
\seq_gset_from_clist:Nn \g_ctuthesis_months_czech_seq { ledna, \'unora, b\v rezna, dubna, kv\v etna, \v cervna,
	\v cervence, srpna, z\'a\v r\'i , \v r\'i jna, listopadu, prosince }

\seq_gset_from_clist:Nn \g_ctuthesis_Months_czech_seq { Leden, \'Unor, B\v rezen, Duben, Kv\v eten, \v Cerven,
	\v Cervenec, Srpen, Z\'a\v r\'i , \v R\'i jen, Listopad, Prosinec }

\seq_gset_from_clist:Nn \g_ctuthesis_months_slovak_seq { janu\'ara, febru\'ara, marca, apr\'i la, m\'aja, j\'una,
	j\'ula, augusta, septembera, okt\v obera, novembera, decembera }

\seq_gset_from_clist:Nn \g_ctuthesis_Months_slovak_seq { Janu\'ar, Febru\'ar, Marec, Apr\'i l, M\'aj, J\'un,
	J\'ul, August, September, Okt\v ober, November, December }

\seq_gset_from_clist:Nn \g_ctuthesis_months_english_seq { January, February, March, April, May, June,
	July, August, September, October, November, December }

\seq_gset_eq:NN \g_ctuthesis_Months_english_seq \g_ctuthesis_months_english_seq

\DeclareExpandableDocumentCommand \monthinlanguage { s m } {
	\IfBooleanTF { #1 } {
		\seq_item:cn { g_ctuthesis_Months_\tl_use:c { g_ctuthesis_field_#2language_tl }_seq }
		{ \ctuthesis_field_use:n { month } }
	} {
		\seq_item:cn { g_ctuthesis_months_\tl_use:c { g_ctuthesis_field_#2language_tl }_seq }
		{ \ctuthesis_field_use:n { month } }
	}
}



% Document types and Faculty names in all langauges
\keys_define:nn { ctuthesis } {

	% Make doctype and faculty aliases for xdoctype and xfaculty
	doctype .meta:n = { xdoctype = {#1} },
	faculty .meta:n = { xfaculty = {#1} },

	% Setup doctypes
	xdoctype .meta:n = { xdoctype-#1 },
	xdoctype .groups:n = { dc, nopre, nopost },

	xdoctype-B .meta:n = {
		doctype-english = { Bachelor ~ Project },
		doctype-czech = { Bakalářská ~ práce },
		doctype-slovak = { Bakalárska ~ práca }
	},
	xdoctype-M .meta:n = {
		doctype-english = { Master ~ Thesis },
		doctype-czech = { Diplomová ~ práce },
		doctype-slovak = { Diplomová ~ práca }
	},
	xdoctype-D .meta:n = {
		doctype-english = { Dissertation ~ Thesis },
		doctype-czech = { Disertační ~ práce },
		doctype-slovak = { Dizertačná ~ práca }
	},

	xfaculty .meta:n = { facultynum={#1}, xfaculty-#1, },

	xfaculty-F1 .meta:n = {
		faculty-english = { Faculty ~ of ~ Civil ~ Engineering },
		faculty-czech = { Fakulta ~ stavební },
		faculty-slovak = { Fakulta ~ stavební }
	},
	xfaculty-F2 .meta:n = {
		faculty-english = { Faculty ~ of ~ Mechanical ~ Engineering },
		faculty-czech = { Fakulta ~ strojní },
		faculty-slovak = { Fakulta ~ strojní }
	},
	xfaculty-F3 .meta:n = {
		faculty-english = { Faculty ~ of ~ Electrical ~ Engineering },
		faculty-czech = { Fakulta ~ elektrotechnická },
		faculty-slovak = { Fakulta ~ elektrotechnická }
	},
	xfaculty-F4 .meta:n = {
		faculty-english = { Faculty ~ of ~ Nuclear ~ Sciences ~ and ~ Physical ~ Engineering },
		faculty-czech = { Fakulta ~ jaderná ~ a ~ fyzikálně ~ inženýrská },
		faculty-slovak = { Fakulta ~ jaderná ~ a ~ fyzikálně ~ inženýrská }
	},
	xfaculty-F5 .meta:n = {
		faculty-english = { Faculty ~ of ~ Architecture },
		faculty-czech = { Fakulta ~ architektury },
		faculty-slovak = { Fakulta ~ architektury }
	},
	xfaculty-F6 .meta:n = {
		faculty-english = { Faculty ~ of ~ Transportation ~ Sciences },
		faculty-czech = { Fakulta ~ dopravní },
		faculty-slovak = { Fakulta ~ dopravní }
	},
	xfaculty-F7 .meta:n = {
		faculty-english = { Faculty ~ of ~ Biomedical ~ Engineering },
		faculty-czech = { Fakulta ~ biomedicínského ~ inženýrství },
		faculty-slovak = { Fakulta ~ biomedicínského ~ inženýrství }
	},
	xfaculty-F8 .meta:n = {
		faculty-english = { Faculty ~ of ~ Information ~ Technology },
		faculty-czech = { Fakulta ~ informačních ~ technologií },
		faculty-slovak = { Fakulta ~ informačních ~ technologií }
	},
	xfaculty-KU .meta:n = {
		faculty-english = { Klokner ~ Institute },
		faculty-czech = { Kloknerův ~ ústav },
		faculty-slovak = { Kloknerův ~ ústav },
		facultynum = { KÚ },
	},
	xfaculty-CIIRC .meta:n = {
		faculty-english = { Czech ~ Institute ~ of ~ Informatics, ~ Robotics ~ and ~ Cybernetics },
		faculty-czech = { Český ~ institut ~ informatiky, ~ robotiky ~ a ~ kybernetiky },
		faculty-slovak = { Český ~ institut ~ informatiky, ~ robotiky ~ a ~ kybernetiky },
		facultynum = { CIIRC },
	},
	xfaculty-MUVS .meta:n = {
		faculty-english = { Masaryk ~ Institute ~ of ~ Advanced ~ Studies },
		faculty-czech = { Masarykův ~ ústav ~ vyšších ~ studií },
		faculty-slovak = { Masarykův ~ ústav ~ vyšších ~ studií },
		facultynum = { MÚVS },
	},

}


\endinput


==> ctuth-pkg.tex <==

%!TEX ROOT = ctutest.tex

\ProvidesExplFile{ctuth-pkg.tex}%
	{2016/06/15}{0.1 t1606152353}%MY TIMESTAMP HERE {0.1}
	{"Packages"\space part\space of\space the\space class\space ctuthesis}

% A lot of the code here is not latex3, but rather the good'ol latex2e code. The reason is that
% it heavily depends on l2e packages, and we decided not to mix the code together too much.

\RequirePackage{lmodern}
\RequirePackage[T1]{fontenc}
\RequirePackage{microtype}
\RequirePackage{graphicx}
\RequirePackage{pdfpages}


%%% BABEL -- LANGUAGE HANDLING

% The loading of the languages is a bit wicked, but it works this way. We load the main language once more
% to make it the default one.
\RequirePackage[\seq_use:Nn \g_ctuthesis_languages_seq {,},\g_ctuthesis_field_mainlanguage_tl]{babel}

% Used for setting title, main or second language
\NewDocumentCommand \selectctulanguage { m } {
	\ctuthesis_field_exists:nTF { #1 language }
		{ \exp_args:Nx \selectlanguage { \ctuthesis_field_use_default:nn { #1 language } { } } }
		{ \msg_error:nnx { ctuthesis } { unknown-field } { #1 language } }
}


%%% COLORS, TEXT FLOW

\RequirePackage{xcolor}

% Define the colors, first in monochrome, then in colour.
\ctuifswitch { savetoner } {
	% savetoner: true
	\definecolor { ctublue } { CMYK } { 100, 43, 0, 0 }
	\definecolor { ctulightblue } { RGB }{ 172, 214, 238 }
	\colorlet    { ctubluetext } { ctublue }
	\colorlet    { ctubluerule } { ctulightblue }
	\colorlet    { ctubluedarkbg } { white }
	\colorlet    { ctubluedarkfg } { ctublue!50!black }
	\colorlet    { ctubluedot } { white }%ctulightblue }
	\colorlet    { ctubluebg } { white }
	\colorlet    { ctulstbg } { ctubluebg }
	\colorlet    { ctublueitemi } { ctublue }
	\colorlet    { ctublueitemii } { ctulightblue }
	\colorlet    { ctugray } { gray }
	\definecolor { ctuorange } { Hsb } { 22, 0.5, 1 }
} {
	\ctuifswitch { monochrome } {
		% savetoner: false, monochrome: true
		\definecolor { ctublue } { gray } { 0.8 }
		\definecolor { ctulightblue } { gray } { 0.9 }
		\definecolor { ctubluetext } { gray } { 0.4 }
		\definecolor { ctubluerule } { gray } { 0.4 }
		\definecolor { ctubluedarkbg } { gray } { 0.2 }
		\definecolor { ctubluedarkfg } { gray } { 1 }
		\definecolor { ctubluedot } { gray } { 0.9 }
		\definecolor { ctubluebg } { gray } { 0.95 }
		\definecolor { ctulstbg } { gray } { 0.95 }
		\definecolor { ctublueitemi } { gray } { 0.4 }
		\definecolor { ctublueitemii } { gray } { 0.4 }
		\definecolor { ctugray } { gray } { 0.5 }
		\definecolor { ctuorange } { gray } { 0.9 }
	} {
		% savetoner: false, monochrome: false
		\definecolor { ctublue } { cmyk } { 1, .43, 0, 0 }
		\definecolor { ctulightblue } { cmyk }{ .3, .13, 0, 0 }
		\colorlet    { ctubluetext } { ctublue }
		\colorlet    { ctubluerule } { ctublue }
		\colorlet    { ctubluedarkbg } { ctublue }
		\colorlet    { ctubluedot } { ctulightblue }
		\colorlet    { ctubluebg } { ctulightblue!50!white }
		\colorlet    { ctulstbg } { ctulightblue!50!white }
		\colorlet    { ctublueitemi } { ctublue }
		\colorlet    { ctublueitemii } { ctulightblue }
		\colorlet    { ctugray } { gray }
		\definecolor { ctuorange } { cmyk } { 0, .51, 1, 0 }
	}
}

\setlength{\parskip}{0pt plus 1pt}

\setlength{\parindent}{11.2pt}


%%% FRONT MATTER --- TWOCOLUMN HANDLING

% This is a "ToC macro" for the twocolumn context
% Arguments: 1) suffix, 2) ToC name
\cs_new_protected:Nn \ctuthesis_maketoc_twocol:nn {
	% Start the chapter
	\chapter* { #2 }
	% locally make rugged pages
	\begingroup
	\raggedbottom
	% We use this trick to add nothing, but also to make sure that
	% any \addvspace for less than 20pt is going to be ignored.
	\vspace*{-20pt}\addvspace{20pt}
	% call the original \@starttoc
	\@starttoc { #1 }
	\newpage
	\endgroup
}

% Environment for the twocolumn frontmatter. It can appear more times in a row
% and should handle it nicely
\NewDocumentEnvironment{ twocolumnfrontmatterpage } { } {
	% Set the page geometry to the title one (it's a bit wider)
	\ctuthesis_geometry_title:
	\newpage
	\pagestyle{twocol}
	% Start the twocolumn.
	\twocolumn[]\relax
	% We are narrow, so we wanna be sloppy
	\sloppy
	% Chapter behaves differently. Both the [] argument and the star * are ignored.
%	\DeclareDocumentCommand\chapter{ s o m }{\relax
%		% Vertical adjustment
%		\vspace* { -\baselineskip }
%		\nointerlineskip
%		% Zero measure vertical box, the contents are raised by something and typeset
%		\vbox to 0pt{\noindent\leavevmode\smash{\raise6pt\hbox to \linewidth{%
%			% In the first column its right-aligned, in the second left-aligned.
%			% It can't be more than one line.
%			\if@firstcolumn\hfil\fi
%			\color{ctubluetext}\LARGE\bfseries\sffamily##3
%			\if@firstcolumn\else\hfil\fi
%		}}}
%		\everypar{\noindent}
%	}
	\DeclareDocumentCommand\chapter{ s o m }{\relax
		% Compute the vertical adjustment
		\skip_gset:Nn \g_ctuthesis_tempa_skip { - \box_ht:N \strutbox }
		{ \LARGE \skip_gsub:Nn \g_ctuthesis_tempa_skip { \box_ht:N \strutbox + \box_dp:N \strutbox } }
		% Space used if not at the beginning of a column
		\skip_vertical:n { 12pt - \g_ctuthesis_tempa_skip }
		% Add the space below the chapter title to the adjustment
		\skip_gsub:Nn \g_ctuthesis_tempa_skip { 2pt }
		% Vertical adjustment
		\vspace* { \g_ctuthesis_tempa_skip }
		% Zero measure vertical box, the contents are raised by something and typeset
		\noindent \leavevmode
		\hbox_to_wd:nn \linewidth {
			% In the first column its right-aligned, in the second left-aligned.
			% It can't be more than one line.
			\if@firstcolumn\hfil\fi
			\leavevmode\color{ctubluetext}\LARGE\strut\bfseries\sffamily##3
			\if@firstcolumn\else\hfil\fi
		}\par
		\skip_vertical:n { 2pt }
		\everypar{\noindent}
	}
	\DeclareDocumentCommand \tableofcontents {  }{ \ctuthesis_maketoc_twocol:nn { toc } { \contentsname } }
	\DeclareDocumentCommand \listoffigures {  }{ \ctuthesis_maketoc_twocol:nn { lof } { \listfigurename } }
	\DeclareDocumentCommand \listoftables {  }{ \ctuthesis_maketoc_twocol:nn { lot } { \listtablename } }
} {
	\ctuthesis_geometry_plain:
	\clearpage
	\onecolumn
	\pagestyle{plain}
}


%%% LANGUAGES

% For every of the languages below, if it's initialized, add the
% custom captions of the class
\@ifundefined{captionsenglish}{}{\g@addto@macro\captionsenglish{\ctucaptionsenglish}}
\@ifundefined{captionsczech}{}{\g@addto@macro\captionsczech{\ctucaptionsczech}}
\@ifundefined{captionsslovak}{}{\g@addto@macro\captionsslovak{\ctucaptionsslovak}}


%%% GEOMETRY

% The ratios of inner:outer margins
% Needs to be separate as this to make the colon ":" have the right catcode
\cs_new:Nx \ctuthesis_geometry_hmarginratio: {4\string :6}

% Target textwidth is 33*basesize (10pt to 12pt)
\dim_const:Nn \g_ctuthesis_geometry_textwidth_dim { \tl_use:N \g_ctuthesis_fontsize_tl * 33 }

% Text occupies 75% of the height of the page by default, less if layout-short is active
% The vmargin ratio is set here in the same manner as the hmargin one above
\ctuifswitch { layout-short } {
	\dim_const:Nn \g_ctuthesis_geometry_textheight_dim { 1.5\g_ctuthesis_geometry_textwidth_dim }
	\cs_new:Nx \ctuthesis_geometry_vmarginratio: {4\string :3}
} {
	\dim_const:Nn \g_ctuthesis_geometry_textheight_dim { 0.75\paperheight }
	\cs_new:Nx \ctuthesis_geometry_vmarginratio: {5\string :6}
}

% Loading the geometry package.
% Almost the same setting appears again in \ctuthesis_geometry_plain:
\RequirePackage [ a4paper ,
	hmarginratio = \ctuthesis_geometry_hmarginratio: ,
	textwidth = \g_ctuthesis_geometry_textwidth_dim ,
 	textheight = \g_ctuthesis_geometry_textheight_dim ,
	vmarginratio = \ctuthesis_geometry_vmarginratio: , ignoreheadfoot ,
	% Should be at least \baselineskip
	headheight = 16pt ,
	marginparsep = 10pt ,
] { geometry }

% Inner margin is 1in + \oddsidemargin. We wanna preserve this value through all
% the different page geometries
\dim_const:Nn \g_ctuthesis_geometry_innermargin_dim { 1in + \the\oddsidemargin }

% The frontmatter pages are a bit wider
\cs_new_protected:Nn \ctuthesis_geometry_title: {
	\newgeometry {
		% Use the stored innermargin value
		inner = \g_ctuthesis_geometry_innermargin_dim ,
		% Increase the width by 20%, but do not exceed 420pt
		textwidth = \dim_min:nn { 420pt } { 1.2 \g_ctuthesis_geometry_textwidth_dim } ,
	 	textheight = \g_ctuthesis_geometry_textheight_dim ,
		vmarginratio = \ctuthesis_geometry_vmarginratio: ,
		headheight = 16pt ,
		ignoreheadfoot ,
		columnsep=30pt ,
	}
}

\cs_new_protected:Nn \ctuthesis_geometry_plain: {
	\newgeometry {
		% Use the stored innermargin value
		inner = \dim_use:N \g_ctuthesis_geometry_innermargin_dim ,
		% Otherwise it's the same as in \RequirePackage[...]{geometry}
		textwidth = \dim_use:N \g_ctuthesis_geometry_textwidth_dim ,
	 	textheight = \g_ctuthesis_geometry_textheight_dim ,
		vmarginratio = \ctuthesis_geometry_vmarginratio: , ignoreheadfoot ,
		headheight = 16pt ,
		marginparsep = 10pt ,
	}
	% Compute the marginparwidth so that we leave 40pt from the page boundary
	\marginparwidth \dimexpr \evensidemargin + 1in - \marginparsep - 40pt
}

% Re-initialize the geometry
\ctuthesis_geometry_plain:


%%% TITLES

\usepackage{titlesec}
% two basic parameters: the rule width and distance
\newlength \ctu@title@rulewidth
\newlength \ctu@title@rulesep
\setlength \ctu@title@rulewidth {11pt}
\setlength \ctu@title@rulesep {11pt}
% box used all the time
\newbox\ctu@title@box
% macro that boxifies the header and adds the rule
\long\def\ctu@title@boxify#1#2#3#4{
	\sffamily
	\bfseries
	\setbox\ctu@title@box\vbox{\hsize\dimexpr\linewidth-\ctu@title@rulewidth-\ctu@title@rulesep\relax
		\vskip#1
		\raggedright
		#3
		\vskip#2
	}
	#4
	\noindent\begin{tabular}{@{}l@{\hspace*{\ctu@title@rulesep}}l@{}}
		\color{ctubluerule}\rule[-\dp\ctu@title@box]{\ctu@title@rulewidth}{\dimexpr\ht\ctu@title@box+\dp\ctu@title@box}
	&
		\box\ctu@title@box
	\end{tabular}\hspace*{-10pt}
	\par
}
\long\def\ctu@title@boxify@x#1#2#3#4#5{
	\sffamily
	\bfseries
	\setbox\ctu@title@box\vbox{\parskip0pt\hsize\dimexpr\linewidth-\ctu@title@rulewidth-\ctu@title@rulesep\relax
		\vskip#1
		\raggedright
		#4
		\vskip#2
	}
	#5
	\noindent\begin{tabular}{@{}l@{\hspace*{\ctu@title@rulesep}}l@{}}
		\color{ctubluerule}
		\rule
			[\dimexpr\ht\ctu@title@box-#3-#1]
			{\ctu@title@rulewidth}
			{\dimexpr#1+#3}
	&
		\box\ctu@title@box
	\end{tabular}\hspace*{-10pt}
	\par
}
% the part style, very simply organized
\def\ttlh@ctupt#1#2#3#4#5#6#7#8{
	\bool_gset_true:N \g_ctuthesis_title_haspart_bool
	\ctu@title@boxify{#5}{#3}{
		{#1\strut\ifttl@label#2\fi\par}
		\vskip30pt
		{\color{ctubluetext}#4\strut#8\strut\par}
	}{\dp\ctu@title@box\dimexpr\textheight-\ht\ctu@title@box-\baselineskip\relax
	}
}
\def\ttlh@ctuch#1#2#3#4#5#6#7#8{
	% If the chapter is starred, we still want to \chaptermark it, just we use the variant \chapterstarmark.
	\ifttl@label\else\chapterstarmark{#8}\fi
	% If the chapter is starred, we still want it in the ToC.
	\ifttl@label\else\addcontentsline{toc}{chapter}{#8}\fi
	\ctu@title@boxify{#5}{#3}{
		{#1\strut\ifttl@label#2\fi\par}
		\medskip
		{\color{ctubluetext}#4\strut#8\strut\par}
	}{}
}
% The section style, very simply organized, subsection style differs only by a missing check for star variant and mark inclusion
% Comments to the chapter style apply here too.
\def\ttlh@ctus#1#2#3#4#5#6#7#8{
	\ifttl@label\else\sectionstarmark{#8}\fi	
	\ifttl@label\else\addcontentsline{toc}{section}{#8}\fi
	\ctu@title@boxify@x{#5}{0pt}{#3}{ #1{\ifttl@label#2\fi\strut\color{ctubluetext}#8\strut} }{}
}
\def\ttlh@ctuss#1#2#3#4#5#6#7#8{
	\ifttl@label\else\addcontentsline{toc}{subsection}{#8}\fi
	\ctu@title@boxify@x{#5}{0pt}{#3}{ #1{\ifttl@label#2\fi\strut\color{ctubluetext}#8\strut} }{}
}
\def\ttlh@ctusss#1#2#3#4#5#6#7#8{
	\ifttl@label\else\addcontentsline{toc}{subsubsection}{#8}\fi
	\ctu@title@boxify@x{#5}{0pt}{#3}{ #1{\ifttl@label#2\fi\strut\color{ctubluetext}#8\strut} }{}
}
% Modified \ttl@page@ii to use \cleardoublepage instead of some idiocy
\def\ttl@page@ii#1#2#3#4#5#6#7{%
  \ttl@assign\@tempskipa#3\relax\beforetitleunit
  \if@openright
    \cleardoublepage
  \else
    \clearpage
  \fi
  \@ifundefined{ttl@ps@#6}%
    {\thispagestyle{plain}}%
    {\thispagestyle{\@nameuse{ttl@ps@#6}}}%
  \if@twocolumn
    \onecolumn
    \@tempswatrue
  \else
    \@tempswafalse
  \fi
  \vspace*{\@tempskipa}%
  \@afterindenttrue
  \ifcase#5 \@afterindentfalse\fi
  \ttl@assign\@tempskipb#4\relax\aftertitleunit
  \ttl@select{#6}{#1}{#2}{#7}%
  \ttl@finmarks
  \@ifundefined{ttlp@#6}{}{\ttlp@write{#6}}%
  \vspace{\@tempskipb}%
  \cleardoublepage
  \if@tempswa
    \twocolumn
  \fi
  \ignorespaces}
% Part title setting
\bool_new:N \g_ctuthesis_title_haspart_bool
\titleformat \part [ctupt] {\Huge} {{\huge\partname\nobreakspace}\thepart} {0pt} {\huge} [0.6\textheight]
\titlespacing* \part {0pt} {0pt} {0pt}
% Tweak into titlesec to make part number contain \numberline. They did not include it for some reason.
\def\ttl@tocpart{\def\ttl@a{\protect\numberline{\thepart}}}
% Chapter title setting
\titleformat \chapter [ctuch] {\huge} {{\LARGE\chaptertitlename\ }\thechapter} {-0\dp\strutbox} {\LARGE} [40pt]
\titlespacing* \chapter {0pt} {40pt} {15pt}
% Section title setting
\titleformat \section [ctus] {\Large} {\thesection\quad} {14pt} {} [2pt]
\titleformat \subsection [ctuss] {\large} {\thesubsection\quad} {11pt} {} [0pt]
\titleformat \subsubsection [ctusss] {\normalsize} {\thesubsubsection\quad} {10pt} {} [0pt]
% Paragraph title setting: runin, with a dot.
\cs_new:Nn \ctuthesis_title_adddot:n {#1\@addpunct.\ignorespaces}
\titleformat \paragraph [runin] {\normalfont\normalsize\bfseries\sffamily} {\theparagraph} {1em} {\ctuthesis_title_adddot:n}
\titleformat \subparagraph [runin] {\normalfont\normalsize\itshape} {\thesubparagraph} {1em} {\ctuthesis_title_adddot:n}
\titlespacing* \paragraph {0pt} {2.25ex plus 1ex minus .2ex} {1em plus 0.3em minus 0.2em}
\titlespacing* \subparagraph {\parindent} {1.75ex plus 0.5ex minus .2ex} {0.7em plus 0.3em minus 0.15em}

% Subsections are the lowest numbered titles, and also the lowest included in ToC.
\setcounter{secnumdepth}{2}
\setcounter{tocdepth}{2}

% Appendix treatment: Even if a chapter in appendix has a star, it will get a number (letter in this case), since
% once you get any appendix, it doesn't make sense not to number some of them.
% Users can use \chapter** if-need-be to get an unnumbered chapter in appendix, but we think it's ridiculous.
\cs_set_eq:NN \ctuthesis_title_orig_appendix: \appendix
\cs_set_eq:NN \ctuthesis_title_orig_chapter: \chapter
\cs_set_eq:NN \ctuthesis_title_orig_makeschapterhead: \@makeschapterhead
% an \if that is true only after \appendix
\newif\ifctu@app \ctu@appfalse
% The new \appendix
\DeclareDocumentCommand \appendix { s s } {
	\ctu@apptrue
	% Call the old \appendix
	\ctuthesis_title_orig_appendix:
	% If the document has \part division, let's make "Appendices" a part on their own
	\bool_if:NT \g_ctuthesis_title_haspart_bool { 
		% But only make the notice in ToC if * is used
		\IfBooleanTF { #2 } {
			% Two stars: If nothing in ToC, at least put there a space.
			\addtocontents{toc}{\vskip 2ex plus 0.2pt}
		} {
			\IfBooleanTF { #1 } {
				% One star: Only add "Appendices" in ToC
				\cleardoublepage
				\addcontentsline { toc } { part } { \appendicesname }
			} {
				% Zero stars: Make "Appendices" page (will be in ToC implicitly
				\part*{ \appendicesname }
			}
		}
	}
	% \chapter ignores one star, so that things like {thebibliography} are numbered
	\DeclareDocumentCommand \chapter { s } { \ctuthesis_title_orig_chapter: }
	% another \appendix will generate a warning and be silently ignored
	\DeclareDocumentCommand \appendix { s s } {
		\msg_warning:nn { ctuthesis } { appendix-twice }
	}
}

\msg_new:nnn { ctuthesis } { appendix-twice } { The~macro~ \token_to_str:N \appendix\ should~
	be~used~only~once.~Silently~ignoring. }


%%% TABLE OF CONTENTS, LISTS OF FIGURES AND TABLES

% Right margin in TOC, note that it need not be wider than the page numbers, so we're fine with 1em.
\def\@tocrmarg{1em}

% New dottedtocline, differs from the default by having numberline variable-width and accomodating to the number
\def\ctu@dottedtocline#1#2#3#4#5{\ifnum #1>\c@tocdepth \else
	\addvspace{0pt plus .2pt}
	{
	\leftskip #2\relax
	\rightskip\dimexpr\@tocrmarg plus 1fil
	\parfillskip -\rightskip
	\parindent #3\relax
	\@afterindenttrue
	\interlinepenalty\@M
	\leavevmode
	\null
	\nobreak
	\hskip -\leftskip
	\def\numberline##1{##1\ }
	{#4}
	\nobreak
	\leaders \hbox {$\m@th \mkern 2mu\hbox {.}\mkern 2mu$}\hfill
	\nobreak
	{\kern0.5em#5}
	\par
	}
\fi}

% Part in ToC: centered, with no pagenumber, bf sf, and with nice space above.
\def\l@part#1#2{
	\addvspace{2ex plus .2pt}
	{
	\centering
	\@afterindenttrue
	\interlinepenalty\@M
	\leavevmode
	\null
	\nobreak
	\def\numberline##1{\partname \nobreakspace ##1\\}%
	\sffamily \bfseries
	#1
	\par
	}\penalty10000\relax
}
% Chapter in ToC: bf sf, no leaders, completely left-aligned, the numberline is variable-width,
% nice space above the chapter line
\def\l@chapter#1#2{
	\addvspace{1ex plus .2pt}
	{
	\raggedright
	\rightskip\dimexpr\@tocrmarg plus 1fil
	\parfillskip -\rightskip
	\@afterindenttrue
	\interlinepenalty\@M
	\leavevmode
	\null
	\nobreak
	\def\numberline##1{##1\hspace*{0.5em}}
	\sffamily \bfseries
	#1
	\nobreak
	\hfill
	\nobreak
	{\kern0.5em#2}
	\par
	}\penalty9999\relax
}
% The section and lower in Toc. We hope nobody would put `\paragraph`s in ToC
\def\l@section{\ctu@dottedtocline{1}{0.6em}{0em}}
\def\l@subsection{\ctu@dottedtocline{2}{1.2em}{0.6em}}
\def\l@subsubsection{\ctu@dottedtocline{3}{1.8em}{1.2em}}
% Figures and tables in LoF and LoT exactly as sections, just the level is set to -2 so that they're always shown
\def\l@figure{\ctu@dottedtocline{-2}{0.6em}{0em}}
\let\l@table\l@figure


%%% FANCY HEADERS

\RequirePackage{fancyhdr}

% Spacial pagestyle for twocolumnpages in the frontmatter: includes centered pagenumber in the bottom
% and we abuse \fancyhead[C] to include the dividing rule
\fancypagestyle{twocol}{
	\fancyhf { }
	\fancyfoot [ RO, LE ] { \texttt { \ctufield { preprint } } }
	\fancyfoot [ C ] { \thepage }
	\fancyhead [ C ] {
		\leavevmode
		\smash {
			\color{ctubluerule}
			\rule [ \dimexpr - \textheight - \headsep - 6pt ]{ 11pt }{ \textheight } 
		}
	}
	\renewcommand { \headrulewidth } { 0pt }
	\renewcommand { \footrulewidth } { 0pt }
	\dim_set_eq:NN \headwidth \textwidth
}

\fancypagestyle { cleardoublepage } {
	% On \cleardoublepage (without star), we want the page number, but nothing else,
	% that is, the same as plain pagestyle
	\ps@plain
}

% Plain pagestyle for chapter and part titles: no rules, just the page number
\fancypagestyle { plain } {
	\fancyhf { }
	\fancyfoot [ RO, LE ] { \texttt { \ctufield { preprint } } }
	\fancyfoot [ C ] { \thepage }
	\renewcommand \headrulewidth { 0pt }
	\renewcommand \footrulewidth { 0pt }
	% reset headwidth to the global textwidth
	\dim_set_eq:NN \headwidth \g_ctuthesis_geometry_textwidth_dim
}

% Headings pagestyle for standard text pages
\fancypagestyle { headings } {
	% Copy the plain pagestyle
	\ps@plain
	% Include the left/rightmark and leaders
	\fancyhead [ LE ] { \ctuthesis_fancy_xlap:nn { right } { \leftmark \ctuthesis_fancy_leaders:n { l } } }
	\fancyhead [ RO ] { \ctuthesis_fancy_xlap:nn { left } { \ctuthesis_fancy_leaders:n { r } \rightmark } }
}

% The leaders macro for the fancyhead: nice little boxes. We make three of them: left, right and center-aligned

\box_new:N \g_ctuthesis_fancy_bluerule_l_box
\hbox_set_to_wd:Nnn \g_ctuthesis_fancy_bluerule_l_box { 10.5pt } {
	{ \color{ctubluedot} \smash{\fontsize{28.88}{0}\fontfamily{lmss}\bfseries.} }
	\hfil
}

\box_new:N \g_ctuthesis_fancy_bluerule_r_box
\hbox_set_to_wd:Nnn \g_ctuthesis_fancy_bluerule_r_box { 10.5pt } {
	\hfil
	{ \color{ctubluedot} \smash{\fontsize{28.88}{0}\fontfamily{lmss}\bfseries.} }
}

\box_new:N \g_ctuthesis_fancy_bluerule_c_box
\hbox_set_to_wd:Nnn \g_ctuthesis_fancy_bluerule_c_box { 10.5pt } {
	\hfil
	{ \color{ctubluedot} \smash{\fontsize{28.88}{0}\fontfamily{lmss}\bfseries.} }
	\hfil
}

% The leaders macro for the fancyhead: nice little boxes,
% the parameter #1 chooses one of the boxes above
\cs_new_protected:Nn \ctuthesis_fancy_leaders:n {
	\hspace*{-1pt}
	\leaders \box_use:c {g_ctuthesis_fancy_bluerule_#1_box} \hfill
	\hspace*{-1pt}
}

% This macro works as follows: The width of the material is actually zero. We use \hbox_overlap_left/right
% to make the headers as wide as we wish, the direction is in #1. In #2 is the contents, and we suppose
% that it contains \ctuthesis_fancy_leaders: and \left/rightmark in desired order; it's typeset gray sf it
\cs_new_protected:Nn \ctuthesis_fancy_xlap:nn {
	\color{ctugray} \sffamily\itshape
	\leavevmode \use:c { hbox_overlap_#1:n } {
		\hbox_to_wd:nn { \paperwidth - 1in - \evensidemargin + 1em } { #2 }
	}
}

% We rename the original \mark... commands and disable them; we do it ourselves
\cs_set_eq:NN \ctuthesis_fancy_markboth_orig:nn \markboth
\cs_set_eq:NN \ctuthesis_fancy_markright_orig:n \markright
\let\markboth\@gobbletwo
\let\markright\@gobble

% New chapter and section marks with no \MakeUppercase
\renewcommand \chaptermark [1] { \ctuthesis_fancy_markboth_orig:nn { \thechapter.\ #1 }{ \thechapter.\ #1 } }
\renewcommand \sectionmark [1] { \ctuthesis_fancy_markright_orig:n { \thesection.\ #1 } }

% Newly defined \chapter/sectionstarmark to be used with unnumbered chapters and sections.
% Not that we like unnumbered ones, but if they need to be there, they sould be in headings, too.
\newcommand \chapterstarmark [1] { \ctuthesis_fancy_markboth_orig:nn { #1 } { #1 } }
\newcommand \sectionstarmark [1] { \ctuthesis_fancy_markright_orig:n { #1 } }

% Better \cleardoublepage that takes proper treatment of the empty pages.
% The starred variant leaves the empty page inbetween really completely empty
\DeclareDocumentCommand \cleardoublepage { s } {
	\clearpage
	\if@twoside\ifodd\c@page\else
%		\IfBooleanTF { #1 } {
			% Starred variant: completely empty page
			\leavevmode
			\thispagestyle{empty}
%		} {
			% Non-starred variant: include page number
			\leavevmode
			\thispagestyle{cleardoublepage}
%		}
		\newpage
		% In twocolumn, we need \newpage twice
		\if@twocolumn\hbox{}\newpage\fi
	\fi\fi
}


%%% FLOATS

\usepackage{float,caption}
% default placement of all floats is `t`
\floatplacement{figure}{t}
\floatplacement{table}{t}
\floatplacement{figure*}{t}
\floatplacement{table*}{t}
% minimum 70% of page height on float pages
\renewcommand{\floatpagefraction}{0.7}
% 2 floats on top, no on bottom
\setcounter{topnumber}{2}
\setcounter{bottomnumber}{0}
\setcounter{totalnumber}{4}
% up to 90% of floats on a mixed page, at least 7% of text
\renewcommand{\topfraction}{0.7}
\renewcommand{\bottomfraction}{0.7}
\renewcommand{\textfraction}{0.2}
% float caption: justification with extra margins on both sides
\DeclareCaptionJustification{myjustify}{\leftskip.8em \rightskip.8em \parfillskip.8em plus 1fil}
% float caption: special format
\DeclareCaptionFormat{myformat}{%
  % float name bf sf
  \begingroup\sffamily\bfseries#1#2:~\endgroup
  % float caption normal font
  \begingroup#3\par\endgroup
}
\DeclareCaptionFormat{mysubformat}{%
  % float name small caps
  #1#2 %
  % float caption normal font
  \begingroup#3\par\endgroup
}
% plain float style is what we like, with captions at the bottom
\floatstyle{plain}
% restyle already existing floats
\restylefloat{figure}
\restylefloat{table}
% set up the captions: no indent of captions, no seperator (seperator is handled by {myformat})
\captionsetup{format=myformat,indent=0pt,labelsep=none,justification=myjustify,font={small},position=below}
% float-caption distance
\abovecaptionskip 8pt plus 3pt minus 1pt
% graphics allowed: pdf, png, jpg
\DeclareGraphicsExtensions{.pdf,.png,.jpg}
% floats should be centered by default:
\g@addto@macro{\@floatboxreset}{\centering}
% nice table rules
\usepackage{booktabs}
\newcommand \Midrule { \midrule[\heavyrulewidth] }
% colored tables
\newenvironment{ctucolortab}{\begin{lrbox}{0}}{\end{lrbox}\ht0\dimexpr\ht0 + 2pt\relax{\fboxsep0pt\colorbox{ctubluebg}{\usebox{0}}}}
\newenvironment{ctucolortab*}{\begin{lrbox}{0}}{\end{lrbox}{\fboxsep0pt\colorbox{ctubluebg}{\usebox{0}}}}


%%% LISTS

% Temp box
\box_new:N \g_ctuthesis_tempa_box
% Macro used to generate the itemize labels
% parameters 1:depth, 2: raise (without ex), 3: scale, 4:color
\cs_new_protected:Nn \ctuthesis_list_prepare_labelitem:nnnn {
	% Each label stored in a box
	\box_new:c { g_ctuthesis_list_label_#1_box }
	% use the temp box to measure the symbol
	\hbox_gset:Nn \g_ctuthesis_tempa_box {
		\scalebox{#3}{\fontfamily{lmss}\bfseries\color{#4}.}
	}
	% The label is actually a shifted up, scaled, coloured lmss bf dot
	\hbox_gset:cn { g_ctuthesis_list_label_#1_box } {
		\box_move_up:nn { #2 ex } \hbox_to_wd:nn {
			\box_ht:N \g_ctuthesis_tempa_box
		} {
			\hss
			\scalebox{#3}{\fontfamily{lmss}\bfseries\color{#4}.}
			\hss
		}
	}
	\cs_set:cpn { labelitem #1 } { \box_use:c { g_ctuthesis_list_label_#1_box } }
}
% The four labels for itemize
\ctuthesis_list_prepare_labelitem:nnnn { i } { 0.18 } { 3.6 } { ctublueitemi }
\ctuthesis_list_prepare_labelitem:nnnn { ii } { 0.18 } { 3.6 } { ctublueitemii }
\ctuthesis_list_prepare_labelitem:nnnn { iii } { 0.36 } { 2.4 } { black }
\ctuthesis_list_prepare_labelitem:nnnn { iv } { 0.48 } { 1.2 } { black }

% Macro for making the box with lmss bf dot "." scaled to the size of \strutbox
% #1 is the width of the box (relative to the width of the resulting dot) and
% #2 is the color of the box
\cs_new_protected:Nn \ctuthesis_list_enumdot:nn {
	\hbox_to_wd:nn { #1\ht\strutbox + #1\dp\strutbox } {
		\hss
		\raisebox{-\dp\strutbox}{
			\resizebox{!}{\dimexpr\ht\strutbox+\dp\strutbox}{
				\fontfamily{lmss}\bfseries\color{#2}.
			}
		}
		\hss		
	}
}

% \itembox takes 5 parameters.
% (#1)(#2) are the left and right padding
% [#3][#4] are the box color and text color
% #5 is the text
\DeclareDocumentCommand \itembox { D(){0.15em} D(){0.15em} >{\TrimSpaces}O{ctubluebg} >{\TrimSpaces}O{black} >{\TrimSpaces}m } {
	\ooalign{
		\hfil \ctuthesis_list_enumdot:nn {1} {#3}
	\cr
		\ctuthesis_list_enumdot:nn {1} {#3} \hfil
	\cr
		\skip_horizontal:n { 0.34\ht\strutbox + 0.34\dp\strutbox }
		\cleaders \ctuthesis_list_enumdot:nn {0.34} {#3} \hfil
		\skip_horizontal:n { 0.34\ht\strutbox + 0.34\dp\strutbox }
	\cr
		\hfil
		\hbox:n { \hspace{#1} { \color{#4} #5 } \hspace{#2} }
		\hfil
	}
}

% Redefine the enumerate labels. The first two levels are boxed,
% the other two are not.
%\def\labelenumi{{\normalfont\itembox[ctubluedarkbg][white]{\bfseries\theenumi.}}}
\def\labelenumi{{\normalfont\itembox{\theenumi.}}}
\def\labelenumii{{\normalfont\itembox(0.1em)(0.1em){\theenumii.}}}
\def\labelenumiii{{\normalfont(\theenumiii)}}
\def\labelenumiv{{\normalfont(\theenumiv)}}

\leftmargini22.2pt
\labelsep6pt


%%% MATH, THEOREMS

\usepackage{amsmath,amssymb,amsfonts}

% Optional loading of amsthm
\ctuthesis_if_switch:nT { pkg-amsthm } {

	\usepackage{amsthm}

	% Redefine standard styles: plain is slanted, definition is normal, note has an italic head (like proof)
	\newtheoremstyle{plain}{3pt plus 1pt}{3pt plus 1pt}{\slshape}{}{\bfseries\sffamily}{.}{.5em}{}
	\newtheoremstyle{plainit}{3pt plus 1pt}{3pt plus 1pt}{\slshape}{}{\bfseries\sffamily}{.}{.5em}{}
	\newtheoremstyle{definition}{3pt plus 1pt}{3pt plus 1pt}{}{}{\bfseries\sffamily}{.}{.5em}{}
	\newtheoremstyle{note}{3pt plus 1pt}{3pt plus 1pt}{}{}{\itshape}{.}{.5em}{}

	% Default style: plain
	\theoremstyle{plain}
	
	% We redefine proof to include a more reasonable spacing above it.
	\DeclareDocumentEnvironment { proof } { O{\proofname} } {
		\par
		\pushQED{\qed}
		\normalfont \topsep0pt plus 1pt
		\trivlist
		\item[
			\hskip\labelsep
		    \itshape
			#1\@addpunct{.}
		]
		\ignorespaces
	}{
		\popQED\endtrivlist\@endpefalse
	}

}	


%%% INDEX

\ctuthesis_if_switch:nT { pkg-makeidx } {

	% Initialize makeindex
	\usepackage{makeidx}
	\makeindex

	% We use multicol rather than twocolumn for the index
	\usepackage{multicol}
	
	% Redefine the index environment to just make the header and start the multicols* envrionment
	% (starred because we don't want to balance the columns), then redefine \item as in original theindex
	\DeclareDocumentEnvironment { theindex } { } {
		\chapter* {\indexname }
		\begin{multicols*}{2}
		\let\item\@idxitem
		% Do not put index sections in ToC. We save the tocdepth and set it to zero, only to restore it after.
		\addtocontents{toc}{\protect\ctu@savetocdepth}
		\addtocontents{toc}{\protect\setcounter{tocdepth}{0}}
		% Inside index, the sections are tighter together
		\titlespacing*\section{}{10pt}{4pt}
	} {
		\addtocontents{toc}{\protect\ctu@restoretocdepth}
		\end{multicols*}
		\clearpage
	}
	
	% How does this work: in \ctu@tocdepth we save the current tocdepth
	\newcommand\ctu@savetocdepth{\xdef\ctu@saved@tocdepth{\the\c@tocdepth}}
	% This macro restores the saved value.
	\newcommand\ctu@restoretocdepth{\global\c@tocdepth\ctu@saved@tocdepth\relax}
}


%%% LISTINGS

\ctuthesis_if_switch:nT { pkg-listings } {
	\RequirePackage{listings}
	\lstset{
		backgroundcolor = \color{ctubluebg},
		basicstyle = \ttfamily,
		columns = fullflexible,
		keepspaces = true,
		tabsize = 4,
%		frame = leftline,
%		framesep = 0pt,
%		framexleftmargin = 3pt,
%		framerule = 0.667pt,
%		rulecolor = \color{ctubluerule},
		frame = single,
		framesep = 0pt,
		framexleftmargin = 2pt,
		framerule = 2pt,
		rulecolor = \color{ctubluebg},
		framexrightmargin = 2pt,
		xleftmargin = 4pt,
		xrightmargin = 4pt,
	}
	\cs_new_eq:NN \ctuthesis_lst_orig_lstinline:w \lstinline
	\newsavebox \ctuthesis_lst_box
	\newcommand* \ctulstsep {0.2em}
	\DeclareDocumentCommand \ctuthesis_lst_do_ctulstinline:nnw { m m m v } {
		\leavevmode
		\microtypesetup{activate=false}
		\begin{lrbox}{\ctuthesis_lst_box}
		\ctuthesis_lst_orig_lstinline:w[#2]#3#4#3
		\end{lrbox}
		\str_if_eq:xnTF {#1} {none}
			{{ \hbox:n {\strut\hspace*{\ctulstsep}\box\ctuthesis_lst_box\hspace*{\ctulstsep}} }}
			{{ \fboxsep0pt\colorbox{#1} {\strut\hspace*{\ctulstsep}\box\ctuthesis_lst_box\hspace*{\ctulstsep}} }}
		\microtypesetup{activate=true}
	}
	\DeclareDocumentCommand \ctulst { D(){\g_ctuthesis_ctulstbg_tl} O{} m } {
		\ctuthesis_lst_do_ctulstinline:nnw { #1 } { #2 } { #3 } #3
	}
	\DeclareDocumentCommand \ctulstbr { D(){ctulstbg} O{} m } {
		\leavevmode
		\begin{lrbox}{\ctuthesis_lst_box}
		\ctuthesis_lst_orig_lstinline:w[#2]{#3}
		\end{lrbox}
		\colorbox{#1}{\box\ctuthesis_lst_box}
	}
}


%%% HYPERREF

\ctuifswitch { pkg-hyperref } {
	\usepackage[
		pdfpagelayout=TwoPageRight, % Correct twopage layout with recto on the right
	]{hyperref}
	% Links with orange borders, in ToC only the page is linked
	\hypersetup{
		colorlinks=false,
		linktocpage=true,
		allbordercolors=ctuorange,
	}
	% Prepare PDFinfo
	\tl_new:N \g_ctuthesis_hyperref_pdfinfo_tl
	\tl_set:Nx \g_ctuthesis_hyperref_pdfinfo_tl {
		pdfinfo = {
			Title = \ctuthesis_field_use:nn { title } { title },
			Author = \ctuthesis_field_use:n { author },
		}
	} 
	\exp_args:NV \hypersetup \g_ctuthesis_hyperref_pdfinfo_tl
}{}

%\ctuifswitch { pkg-hyperref } {
%	\hypersetup{colorlinks=false,linktocpage=true,linkbordercolor=0 122 195}
%}


%%% VARIOUS TWEAKS

% Provide \phantomsection and \texorpdfstring to make them available in case hyperref wasn't loaded
\providecommand\phantomsection{}
\providecommand\texorpdfstring[2]{#1}
% Provide \microtypesetup to make it available in case microtype wasn't loaded
\providecommand\microtypesetup[1]{}


\endinput


==> ctuth-templates.tex <==

%!TEX ROOT = ctutest.tex

\ProvidesExplFile{ctuth-templates.tex}%
	{2016/06/15}{0.1 t1606152353}%MY TIMESTAMP HERE {0.1}
	{"Templates"\space part\space of\space the\space class\space ctuthesis}

% The titlepage, includes doctype, faculty, department, title, author,
% and some auxiliary information at the bottom
\ctutemplateset{titlepage}{
	\thispagestyle { empty }
	\noindent
	\vbox to \textheight{%
	% The titlepage goes all way up to the header (taking one \baselineskip of the head)
	\vspace*{\dimexpr-\baselineskip-\headsep}
	\vss%
	{\noindent\leavevmode\color{ctubluerule}\vrule width 11pt\hspace*{11pt}}
	% The main vbox of the titlepage is larger by (bls + heasep) up and (footskip) down
	\vbox to \dimexpr\textheight + \baselineskip + \headsep + \footskip{
		% Reduce hsize by the rule width and the sep
		\hsize\dimexpr\linewidth-17pt
		% No justification, sf bf font
		\raggedright \sffamily \bfseries
		\selectctulanguage{title}
		%
		% The document type
		{\ctufield[title]{doctype}\par}
		%
		\vspace*{3ex}
		%
		% A table containing: the CTU logo and name, faculty number, faculty and deparment name
		\begin{tabular}{@{}l@{\hspace*{1em}}l@{}}
			\Large\includegraphics[height=\dimexpr4\normalbaselineskip-1ex]{ctu_logo_black}
		&
			\Large\color{ctubluetext}\begin{tabular}[b]{@{}l@{}}\ctufield[title]{university-endl}\end{tabular}
		\\[3ex]
%			\begin{tabular}[c]{@{}l@{}}
			\raisebox{-8pt}{
			\color{ctubluetext}\fontsize{32.7}{32.7}\selectfont
			\setbox0\hbox{\smash{\ctufield{facultynum}}\vphantom{X}}
			\ifdim\wd0>2em \scalebox{0.9}[1]{\textls[-50]{\smash{\ctufield{facultynum}}\vphantom{X}}}\else\box0\fi
			}
%			\end{tabular}
		&
			\begin{tabular}[c]{@{}l@{}}\rlap{\ctufield[title]{faculty}}\\[2pt]\ctufield[title]{department}\end{tabular}
		\end{tabular}\par
		%
		\vspace{8ex plus 1fill}
		%
		% The title, in two languages
		{\LARGE\color{ctubluetext}
		\ctufield[title]{title}
		\par}
		%
		\vspace{3ex}
		%
		{\Large\color{ctubluetext}
		\ctufield[title]{subtitle}
		\par}
		%
		\vspace*{8ex}
		%
		% The author
		{\Large
		\ctufield{author}
		\par}
		%
		\vspace{0pt plus 3fill}
		{
		% The "metadata": supervisor, field of study, month and year
		\parskip 1pt
		\ctuiffield*{supervisor}{\supervisorname :~{\frenchspacing\ctufield{supervisor}}\par}{}
		\ctuiffield*{supervisor-specialist}{\supervisorspecialistname :~{\frenchspacing\ctufield{supervisor-specialist}}\par}{}
		\ctuiffield*[title]{fieldofstudy}{\fieldofstudyname :~\ctufield[title]{fieldofstudy}\par}{}
		\ctuiffield*[title]{subfieldofstudy}{\subfieldofstudyname :~\ctufield[title]{subfieldofstudy}\par}{}
		\monthinlanguage*{title}~\ctufield{year}\par
		}
	}
	\vss
	% The titlepage goes all way down to the foot
	\vspace*{-\footskip}
	}
	\par
}

% This include the specification file, and does nothing more
% \ctutemplateset{include.specification}{
% 	\includepdf[pages=-]{\tl_use:c{ g_ctuthesis_field_specification-file_tl }}
% }

% Includes the specification as a chapter
% \ctutemplateset{specification.as.chapter}{
% 	\cleardoublepage
% 	% If it is an appendix, it gets a number, if not, it does not
% 	\ifctu@app
% 		\refstepcounter{chapter}
% 		\phantomsection
% 		\addcontentsline{toc}{chapter}{\protect\numberline{\thechapter}\specificationname}
% 	\else
% 		\phantomsection
% 		\addcontentsline{toc}{chapter}{\specificationname}
% 	\fi
% 	\ctutemplate{include.specification}
% }

\ctutemplateset{twocolumn.abstract.in.titlelanguage}{
		\selectctulanguage{title}
		\chapter{\abstractname}\noindent
		\ctufield[title]{abstract}\par
		{ \raggedright
		\paragraph{\keywordsname :}
		\ctufield[title]{keywords}
		\paragraph{\supervisorname :}
		\ctuiffield*{supervisor}{
			\ctufield{supervisor}
			\ctuiffield*{supervisor-address}{
				\\
				\ctufield{supervisor-address}
			}{}
		}{}
		\par }
}

\ctutemplateset{twocolumn.abstract.in.secondlanguage}{
		\selectctulanguage{second}
		\chapter{\abstractname}\noindent
		\ctufield[second]{abstract}\par
		{ \raggedright
		\paragraph{\keywordsname :}
		\ctufield[second]{keywords}
		\paragraph{\titletranslationname :}
		\ctufield[second]{title}
		\ctuiffield*[second]{subtitle}{
			\ --- \ \ctufield[second]{subtitle}
		} { }
		\par }
}

\ctutemplateset{twocolumn.tableofcontents}{
		\selectctulanguage{main}
		\tableofcontents
}

\ctutemplateset{twocolumn.thanks}{
		\selectctulanguage{title}
		\chapter{\thanksname}\noindent
		\ctufield{thanks}
}

\ctutemplateset{twocolumn.declaration}{
		\selectctulanguage{title}
		\chapter{\declarationname}\noindent
		\ctufield{declaration}
}

\ctutemplateset{twocolumn.listoffigures}{
		\selectctulanguage{main}
		\listoffigures
}

\ctutemplateset{twocolumn.listoftables}{
		\selectctulanguage{main}
		\listoftables
}

% Abstract template includes the Acknowledgements, Declaration and two Abstracts
% the abstracts are accompanied by the keywords and possibly other information
\ctutemplateset{maketitle.twocolumn.default}{
	\begin{twocolumnfrontmatterpage}
		\ctutemplate{twocolumn.thanks}
	\newpage
		\ctutemplate{twocolumn.declaration}
	\clearpage
		\ctutemplate{twocolumn.abstract.in.titlelanguage}
	\newpage
		\ctutemplate{twocolumn.abstract.in.secondlanguage}
	\clearpage
		\ctutemplate{twocolumn.tableofcontents}
	% The "loft" template is included only if at least one of the lists is enabled
	\bool_if:nTF {
		\ctuthesis_if_switch_p:n { front-list-of-figures }
		|| \ctuthesis_if_switch_p:n { front-list-of-tables }
	} {
		\clearpage
		\ctutemplate{twocolumn.loft}
	} { }
	\end{twocolumnfrontmatterpage}
}

% Lists of Figures and Tables
\ctutemplateset{twocolumn.loft}{
		\ctuifswitch { front-list-of-figures } { \ctutemplate{twocolumn.listoffigures} } { }
	\newpage
		\ctuifswitch { front-list-of-tables } { \ctutemplate{twocolumn.listoftables} } { }
}

% The maketitle command (moreorless): roman page numbering
\ctutemplateset{maketitle}{
	\frontmatter
	% Start with the titlepage
	\ctutemplate{titlepage}
	% title verso is empty (the star makes it completely empty in our template)
	\cleardoublepage*
	% If the specification has to be in front, include it. It it's one page only,
	% the verso is left empty
% 	\ctuifswitch{front-specification}{
% 		\ctutemplate{include.specification}
% 		\cleardoublepage*
% 	} { }
	% The abstract and alike
	\ctutemplate{maketitle.twocolumn.default}
	\def\thepage{}
	% Start the mainmatter
	\mainmatter
}

% Minor change to \mainmatter: we add the star to \cleardoublepage
\DeclareDocumentCommand \mainmatter { } {
	\cleardoublepage*
	\@mainmattertrue
	\pagenumbering{arabic}
	\pagestyle{headings}
}

% \maketitle command itself just calls the maketitle template
\DeclareDocumentCommand \maketitle { } {
	\ctutemplate{maketitle}
}

\endinput
